Certified Program Synthesis with a Multi-Modal Verifier

Certified program synthesis (aka vericoding) is the process of automatically generating a program, its formal specification, and a machine-checkable proof of their alignment from a natural-language description. Two challenges make vericoding difficult. First, specifications synthesised from natural language are often either too weak to be meaningful or too strong to be implementable, yet existing approaches lack systematic means to detect such defects. Second, the landscape of program verifiers is fragmented: each tool supports a particular reasoning mode -- auto-active (e.g., Dafny, Verus) or interactive (e.g., Coq, Lean) -- with its own trade-off between automation and expressivity. This forces every synthesis methodology to be tailored to a single verification paradigm, limiting the class of tasks it can handle effectively. We overcome both challenges by structuring the certified synthesis workflow around a multi-modal verifier -- a single tool combining dynamic validation, automated proofs, and interactive proof scripting in one foundational framework. We realise this idea in LeetProof, an agentic pipeline built on Velvet, a multi-modal verifier embedded in Lean. Multi-modality enables LeetProof to validate generated specifications via randomised property-based testing before any code is synthesised, decompose the synthesis task into sub-problems guided by verification conditions, and delegate residual proof obligations to frontier AI provers specialised for Lean. We evaluate LeetProof on benchmarks derived from prior work on certified synthesis. Our specification validation uncovers defects in existing reference benchmarks, and LeetProof's staged pipeline achieves a significantly higher rate of fully certified solutions than a single-mode baseline at the same budget -- consistently across two frontier LLM backends.

==> design.tex <==

\section{\tool Agent Design}
\label{sec:design}

\todo{ Here we can indtroduce multiple agents and explain their roles. I've put down a few, please, expand}


\subsection{Specification Agent}
\label{sec:spec}

Here, we explain Validation Sepcifications by Symbolic Testing

\subsection{Program Generation Agent}
\label{sec:proggen}

\todo{Explain more}

\subsection{Invariant Generation Agent}
\label{sec:invar-gener-agent}




==> evaluation.tex <==

% **Evaluation**
%
% RQ1 — How well does the generated specification capture the intent of the natural language? (This shows we are not proving trivial statements.)
% - Implicit oracle: the postcondition uniquely determines the output.
% - We judge that by comparing with the Verina benchmark. We ask Aristotle to prove the equivalence of our & Verina's specification
%
% RQ2 — Does staging of program synthesis by using a program logic that allows us to add an invariant filtering states improve **overall synthesis pipeline success rates** (compared to not having invariant filtering)?
% - RQ2' — Is the success rate maintained when switching the LLM model?
%
% imperative programs
% - with Velvet synthesises 27/50
% - with Lean synthesises 18/50
%
% -> are there problems that Lean solves and Velvet doesn't and vice-versa?
%
% RQ3 — How many fully invariant-annotated programs that passed all filters (i.e. failed at the last stage of the pipeline = the proving stage) are provable if more resources are dedicated to proving (using Aristotle)?
%
% - 15 Velvet programs passed all filters, but had only partial proofs; all those were discharged by Aristotle
% - 26 type-correct Lean programs could not be proven; 22 of those were discharged by Aristotle, and 4 of them Aristotle couldn't prove
%
% RQ4 — How effective at filtering bad candidates is each respective stage of the pipeline? (Ablation.)

\section{Evaluation}
\label{sec:evaluation}

Our evaluation investigates the following research questions.

\subsection{RQ1: Specification Accuracy}
\label{sec:rq1}
\begin{rqbox}
\textbf{RQ1}: How well does the generated specification capture the intent of the natural language description?
\end{rqbox}
To evaluate the accuracy of generated specifications, we use the Verina benchmark, which provides natural language problem descriptions paired with manually curated formal specifications. For each problem, we run our specification generator to produce a candidate specification $(\mathit{pre}_{\text{gen}}, \mathit{post}_{\text{gen}})$ and compare against the reference $(\mathit{pre}_{\text{ref}}, \mathit{post}_{\text{ref}})$. We assess semantic accuracy via formal equivalence checking in Lean~4. Concretely, we encode the following proof obligations in Lean: (i) the preconditions are equivalent, $\mathit{pre}_{\text{gen}} \leftrightarrow \mathit{pre}_{\text{ref}}$, and (ii) for all inputs satisfying the precondition, the postconditions are equivalent, i.e., $\mathit{pre}_{\text{gen}} \rightarrow (\mathit{post}_{\text{gen}} \leftrightarrow \mathit{post}_{\text{ref}})$. We discharge these obligations using \aristotle. When equivalence cannot be established, we manually inspect the specifications to categorize the discrepancies.

Evaluation of the 188 problems yields the following breakdown:
\begin{itemize}
    \item \textbf{Equivalent (149):} Generated specifications are logically equivalent to the references.
    
    \item \textbf{Potential Issues in Reference Specifications (16):} We identified inconsistencies between the benchmark's reference postconditions and intended semantics.

    \item \textbf{Acceptable Precondition Variations (14):} Preconditions differ slightly (e.g., admitting broader input domains than the prompts specified) but remain valid semantic extensions. For example, in \texttt{advanced\_53} (minimum right shifts to sort a list), the prompt specifies positive elements, while the reference precondition admits all natural numbers. These variations are immaterial to the core logic.

    \item \textbf{Ambiguous Natural Language (3):} Vague descriptions admit multiple reasonable interpretations, leading to divergent but defensible specifications. For example, in \texttt{advanced\_45} (maximum subarray sum), the prompt does not specify whether a valid subarray can be empty.
    
    \item \textbf{Over-restrictive Postconditions (2):} Our postconditions impose unstated constraints to ensure determinism. For example, in \texttt{advanced\_76}, the generated specification enforces a specific tie-breaking rule that is not mandated by the original problem description.
    
    \item \textbf{Incorrect Specifications (3):} The generated specifications are semantically inconsistent with the problem description, comprising incorrect preconditions (2 cases) and an incorrect postcondition (1 case).
    
    \item \textbf{Incomparable (1):} One problem (\texttt{basic\_104}) could not be evaluated because the reference specification relies on a custom data structure.
\end{itemize}

The over-restrictive cases stem from a preference for deterministic specifications. Including the incorrect cases, our approach deviates from the intended semantics in only 5/188 instances (2.7\%). Notably, this deviation rate is lower than the inconsistency rate of the human-written benchmark itself (16/188, or 8.5\%), underscoring the reliability of our automated generation.

Notably, the specification-level PBT techniques described in Section~\ref{sec:spec-pbt} play a critical role in improving specification quality. During the above evaluation, PBT identified errors in two specifications that had already passed the LLM judge, reducing the number of incorrect specifications from 7 (3.7\%) to 5 (2.7\%). In addition, PBT uncovered one case where the generated test cases, despite passing the LLM judge, did not satisfy the stated preconditions.

Beyond this evaluation, we further apply specification-level PBT to the specifications in both Verina and Clever. We use the test cases provided by the benchmarks. For problems with reference implementations, we additionally attempt to sample a batch of inputs satisfying the preconditions and obtain outputs by executing the implementations. Without any assistance from LLMs, this process uncovers 13 issues in Verina and 18 in Clever within one day on a single Apple M4 Pro machine (14-core CPU, 24 GB RAM). 

Worth noting is that specification-level PBT is significantly more cost-effective than LLM-based judging to find the specification issues. For the 13 issues identified by PBT in Verina, PBT requires only 9 minutes in total, whereas using \aristotle for equivalence checking takes approximately 8 hours.

Across the two sets of experiments, we identify a total of 16 issues in Verina, and 18 in Clever. Table~\ref{tab:spec-issues} summarizes the discovered issues. We have reported all of them to the benchmark authors. For Verina, 15 issues have been confirmed and fixed, while the remaining one is still under review. All 18 issues in Clever are currently pending review.

\input{figures/spec_issues_table}

\subsection{Benchmark Building for RQ2-RQ4}
\label{sec:benchmark}

We construct a new benchmark tailored for vericoding evaluation. While existing benchmarks such as Verina provide curated specifications and support reasoning from natural language to formal specifications, they are not well-suited for our purpose for several reasons. First, the problem distribution tends to favor functional programming styles. Only relatively few tasks involving imperative patterns such as two-pointer techniques or algorithms requiring frequent random index access over arrays. Second, these benchmarks typically do not enforce time and space complexity constraints, allowing trivial implementations that satisfy correctness but do not reflect realistic efficiency requirements. Third, some benchmarks have been publicly available for an extended period, and their reference Lean implementations may have been incorporated into the training data of underlying LLMs.

During development, we manually select 15 imperative-style problems from LeetCode to validate and refine LeefProof. For evaluation, we further sample 35 problems from LeetCode using Anthropic Claude under the following criteria:
(1) inputs consist only of simple data types (integers, arrays, or strings);
(2) problems involving complex data structures (e.g., hash tables, graphs, or balanced binary trees) are excluded;
(3) the problem admits a deterministic input-output specification;
(4) the sampled set includes both classical and relatively recent problems;
(5) the problems are of easy to medium difficulty, according to LeetCode.

For each problem, we ask Anthropic Claude to suggest an time complexity based on the input constraints. We then manually check the correctness of these annotations. For a small number of problems, we perform minor simplifications (e.g., assuming the input is already sorted to avoid sorting), allowing synthesis and verification to focus on the core algorithmic aspects rather than auxiliary dependencies.

In the following sections, we report results on both the development set and the evaluation set, and explicitly distinguish between them when necessary to avoid bias.

\subsection{RQ2: Compare with single-mode Synthesis}
\label{sec:rq2}
\begin{rqbox}
\textbf{RQ2}: Does the multi-model LeetProof show advantage over a single-mode Lean synthesis baseline?
\end{rqbox}

\subsubsection{Experimental Setup}
To evaluate the impact of staged synthesis and verification-guided feedback, we compare our full pipeline against a single-mode Lean synthesis baseline, in which the intermediate Velvet methods and loop invariants are omitted and the LLM directly synthesizes single-mode Lean programs verified by the same prover. Both configurations use GPT-5.2 as the underlying model, identical specifications, and are subject to an equal computational budget of \$5.

\subsubsection{Synthesis Results}

\autoref{tab:synthesis-results} presents the certified synthesis outcomes for both the Velvet-based pipeline and the single-mode Lean baseline. For each problem, we record one of three outcomes:

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/proof_waffle.pdf}
  \caption{Synthesis Outcome}
  \label{tab:synthesis-results}
\end{figure}

\todo{remember to update numbers here}

\paragraph{Fully Proven.}
The pipeline successfully synthesizes an implementation (along with loop invariants, in the case of Velvet synthesis) and produces a complete formal proof of correctness against the specification. Velvet achieves 27 fully proven solutions out of 50 problems, significantly outperforming the single-mode Lean baseline, which produces 18 fully proven solutions.

\paragraph{Partially Proven.}
An implementation (and invariants) is synthesized, but the proof is incomplete. Velvet produces 15 partially proven programs, while single-mode Lean produces 12.

\paragraph{Synthesis Failure.}
No implementation (or invariant) passes the pipeline's verification checks. Velvet encounters 9 synthesis failures, slightly more than the 7 observed in the single-mode Lean baseline. We conjecture that the additional staging in the Velvet pipeline imposes stricter validation, leading to a higher rejection rate at the synthesis stage.

\input{figures/proof_comparison_table}

\paragraph{Overlap Analysis.}
\todo{remember to update numbers here}
\autoref{tab:proof-comparison} breaks down the per-problem overlap between the two pipelines. While Velvet outperforms Lean overall, Velvet does not uniformly dominate single-mode Lean baseline: 2 problems are fully proven by Lean but result in synthesis failure for Velvet, and a further 2 are fully proven by Lean but only partially proven by Velvet. This is to be expected: Velvet is a Dafny-like DSL that targets imperative-style programs, whereas single-mode Lean baseline synthesis targets functional-style programs. Depending on the nature of the problem, one style may yield a more concise implementation whose correctness is easier to establish.

Since Velvet is itself a DSL embedded in Lean, this limitation does not restrict the user. Users can always freely fall back to single-mode Lean baseline synthesis within the same framework, retaining the flexibility to choose the approach best suited to each problem.

\subsection{RQ3: Last-Mile Proof Effort}
\label{sec:rq3}
\begin{rqbox}
\textbf{RQ3} : Are failures in the final proof stage due to incorrect intermediate artifacts or insufficient proof effort? If the latter, how hard is it to complete the proof with additional effort?
\end{rqbox}

\todo{update numbers here}

For partially proven outcomes in RQ2, we further attempt to discharge the remaining verification conditions using \aristotle, in order to distinguish between two failure modes: (i) the synthesized implementation or invariants are incorrect, making the verification conditions unprovable, or (ii) the conditions are in fact provable but were not discharged due to limited prover power or budget.

As shown in \autoref{tab:synthesis-results}, Velvet produces 15 partially proven programs, all of which are subsequently discharged by \aristotle. This demonstrates that the Velvet pipeline successfully synthesizes correct implementations and loop invariants in these cases; the partial proofs reflect limitations in prover power or budget rather than errors in the synthesized artifacts.

The single-mode Lean baseline baseline yields 22 partially proven programs. \aristotle successfully discharges 18 of these, but gives up on the remaining 4. Importantly, for all 4 of these problems, the verification conditions produced by the corresponding Velvet runs are successfully discharged by \aristotle. This suggests that even in partially proven cases, the Velvet pipeline generates proof obligations that are structurally easier to discharge.

\subsection{RQ4: LLM Backend Robustness}
\label{sec:rq4}
\begin{rqbox}
\textbf{RQ4}: Are the effects we discussed in RQ2 and RQ3 consistent across different LLM backends?
\end{rqbox}

To assess whether the findings from RQ2 and RQ3 are robust to the choice of LLM backend, we randomly sample 25 problems from the benchmark and replicate the same experiment using Claude Opus 4.6 in place of GPT-5.2, keeping all other settings identical.

\todo{add results here}

% \subsection{RQ5: Effectiveness of Property-Based Testing}
% \begin{rqbox}
% \textbf{RQ5} [Effectiveness of Property-Based Testing]: How effective is property-based testing at filtering out incorrect candidates?
% \end{rqbox}

% We evaluate the effectiveness of PBT in filtering out incorrect candidates at specification-level and invariant-level.

% \paragraph{Specification-Level PBT.} We evaluate the effectiveness of property-based testing (PBT) for specifications using the logs from RQ1. Notably, in our specification generation workflow, only candidates passing a LLM judge are further tested by PBT.
% Across all Verina benchmark problems, we identify five specifications that are semantically incorrect but passed Judge. Among these, PBT successfully detects two cases with errors in the postconditions. In addition, PBT uncovers one case in which the generated test cases are incorrect, despite passing Judge. This shows that even with the LLM's strong reasoning, PBT remains a valuable complement that catches specification bugs.

% \paragraph{Invariant-Level PBT.} The effectiveness of invariant-level PBT is evaluated using the logs from RQ2. Unlike specification-level PBT, which acts as a comprehensive final guard and may take several minutes per problem, invariant-level PBT serves as a rapid pre-screen to filter out invalid candidates before invoking the LLM judge. Analyzing the logs from RQ2, the pipeline performed XXX rounds of type-checked invariant inference. Of the ZZZ candidates ultimately rejected, PBT successfully filtered out YYY invalid invariants. \todo{remember to add number here}
% Although the absolute detection rate of invariant-level PBT is modest, it provides a critical cost-saving benefit compared to relying exclusively on the LLM judge. We attribute this to two primary factors. First, since invariant generation typically requires many iterations, we cannot afford to allocate substantial time for testing; in practice, PBT is limited to around 30 seconds per candidate. Second, loop invariants often exhibit complex structures, such as deeply nested quantifiers and higher-order predicates. Despite the enhancements to Plausible detailed in Section~\ref{sec:plausible-extensions}, such predicates may still exceed the expressive and testing capabilities of our PBT framework.

==> experiments.tex <==



==> figures/iteration_budget_table.tex <==
\begin{table}[!ht]
\centering
\small
\caption{Maximum iteration budget for each synthesis stage.}
\label{tab:iteration-budget}
\begin{tabular}{lc}
\toprule
\textbf{Stage} & \textbf{Iterations} \\
\midrule
Lean synthesis & 15 \\
Velvet program synthesis & 15 \\
Velvet invariant synthesis & 15 \\
Specification generation & 10 \\
\bottomrule
\end{tabular}
\end{table}


==> figures/pipeline_tikz_styles.tex <==
\providecommand{\llmboticon}{%
	\tikz[baseline=-0.55ex, x=0.85mm, y=0.85mm]{
		\draw[line width=0.35mm, rounded corners=0.5mm]
		(-1.6,-1.2) rectangle (1.6,1.2);
		\draw[line width=0.35mm] (0,1.2) -- (0,2.0);
		\fill (0,2.2) circle (0.22);
		\fill (-0.55,0.2) circle (0.16);
		\fill (0.55,0.2) circle (0.16);
		\draw[line width=0.3mm] (-0.75,-0.45) -- (0.75,-0.45);
		\draw[line width=0.35mm] (-1.6,0) -- (-2.2,0);
		\draw[line width=0.35mm] (1.6,0) -- (2.2,0);
		\draw[line width=0.35mm] (-0.8,-1.2) -- (-0.8,-2.0);
		\draw[line width=0.35mm] (0.8,-1.2) -- (0.8,-2.0);
	}%
}

\tikzset{
	pipeline/base/.style={
			draw=blue!60!black,
			rounded corners=3pt,
			thick,
			align=center,
			inner sep=3pt,
			minimum height=8mm,
			%font inherited from tikzpicture
		},
	pipeline/artifact/.style={
			pipeline/base,
			draw=blue!80!black,
			fill=blue!5
		},
	pipeline/panel/.style={
			draw=blue!60!black,
			rounded corners=4pt,
			thick,
			fill=black!2
		},
	pipeline/step/.style={
			pipeline/base,
			draw=green!60!black,
			fill=green!5,
			minimum width=19mm
		},
	pipeline/llmstep/.style={
			pipeline/base,
			draw=purple!80!black,
			fill=purple!10,
			minimum width=19mm
		},
	pipeline/outcome/.style={
			pipeline/base,
			draw=blue!80!black,
			fill=blue!20
		},
	pipeline/partial/.style={
			pipeline/base,
			draw=orange!70!black,
			fill=orange!10
		},
	pipeline/flow/.style={
			->,
			thick,
			draw=blue!60!black
		},
	pipeline/revise/.style={
			->,
			thick,
			dashed,
			draw=red!70!black
		},
	pipeline/label/.style={
			font=\scriptsize,
			inner sep=1.5pt,
			auto
		},
	pipeline/group/.style={
			draw=green!60!black,
			fill=green!8,
			rounded corners=3pt,
			thick
		}
}


==> figures/total_partial_example.tex <==
\begin{figure*}[t]
  \centering
\hspace{3pt}
  \begin{minipage}[t]{0.49\linewidth}
  \centering
  % \vspace{-100pt}
  % \begin{subfigure}[t]{\linewidth}
  \begin{leancode}
|\hlt{white}{\lw{method} insertionSort (\lw{mut} a: arrInt) \lw{return} (u: Unit)}|
|\hlt{white}{\require 1 $\leq$ size a}|
|\hlt[black][0.6pt]{yellow}{\ensures $\forall$ i j, i $\leq$ j < size a → aNew[i] $\leq$ aNew[j]}|
|\hlt[black][0.6pt]{yellow}{\ensures toMultiset a = toMultiset aNew}|do
  |\hlt{white}{\lw{let} a$_{0}$ := a}|
  |\hlt{white}{\lw{let} \lw{mut} n := 1}|
  |\hlt{white}{\whilel n $\neq$ size a}|
  |\hlt{white}{\invariant n $\leq$ size a}|
  |\hlt[black][0.6pt]{yellow}{\invariant $\forall$ i j, i < j < n → a[i] $\leq$ a[j]}|
  |\hlt[black][0.6pt]{yellow}{\invariant toMultiset a = toMultiset a$_{0}$}|
  |\hlt[black][0.6pt]{red}{\decreasing size a$_{0}$ - n}|do
    |\hlt{white}{\lw{let} \lw{mut} mind := n}|
    |\hlt{white}{\whilel mind $\neq$ 0}|
    |\hlt[black][0.6pt]{yellow}{\invariant mind $\leq$ n}|
    |\hlt[black][0.6pt]{yellow}{\invariant $\forall$ i j, i < j $\leq$ n $\land$ j $\neq$ mind → a[i] $\leq$ a[j]}|
    |\hlt[black][0.6pt]{yellow}{\invariant toMultiset a = toMultiset a$_{0}$}|
    |\hlt[black][0.6pt]{red}{\decreasing mind}|do
      |\hlt{white}{\lw{if} a[mind] < a[mind - 1] \lw{then}}|
        |\hlt{white}{  swap a (mind - 1) mind}|
      |\hlt{white}{mind := mind - 1}|
    |\hlt{white}{n := n + 1}|
 |\lw{prove\_correct}| insertionSort by |\lw{loom\_solve}|
  \end{leancode} 
%\setlength{\abovecaptionskip}{1pt}
%\setlength{\belowcaptionskip}{-10pt}  
  \caption{\velvet code and proof of insertion sort}
  \label{fig:insertion-sort}
  % \end{subfigure}

  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.45\linewidth} 
  \vspace{0.5pt}
  \centering
  % \begin{subfigure}[t]{\linewidth}
  \includegraphics[width=\linewidth]{figures/Infoview.pdf}
  \setlength{\abovecaptionskip}{18pt}
%  \setlength{\belowcaptionskip}{-3pt}  
  \caption{\lean InfoView for a failed termination proof}
  \label{fig:goal-obligation}
  % \end{subfigure}

  \end{minipage}
%  \vspace{-10pt}
% \caption{Insertion sort implementation and corresponding verification goal}
\end{figure*}


==> figures/withdraw_exn_nondet.tex <==
\begin{figure}[t]
  \centering
\hspace{5pt}
  \begin{minipage}[t]{0.48\linewidth}
  \centering
  
  \begin{subfigure}[t]{\linewidth}
  \centering
  \begin{leancode}
|\bdef| withdraw (amounts : List Nat) |\returns| Unit
|\require| balance |$\geq$| amounts.sum
|\ensures| balance + amounts.sum = balanceOld do
  let mut tmp := amounts
  |\whilel| tmp.nonEmpty
  |\invariant| balance    + amounts.sum = 
            balanceOld + tmp.sum 
  |\decreasing| tmp.length do
    let amount := tmp.head
    if amount > balance then |\throw| "Insufficient funds"
    else balance := balance - amount
    tmp := tmp.tail
  \end{leancode}
  \setlength{\abovecaptionskip}{2pt}
  % \setlength{\belowcaptionskip}{-12pt}
  \caption{Withdrawal with exceptions}
  \label{fig:withdraw-exn}
  \end{subfigure}

\vspace{7pt}

  \begin{subfigure}[t]{\linewidth}
  \centering
  \begin{leancode}
|$\mu$| (f : ExceptT |$\alpha$| BankM (Bal → Prop)) := 
  |$\mu$| (m := BankM) do 
    let ex ← (f : BankM (Except |$\alpha$| (Bal → Prop))); 
    |\lw{return}| ex.getD (|$\lambda$| _ => False)
  \end{leancode}
  \setlength{\abovecaptionskip}{2pt}
  \caption{Semantic embedding of exceptions}
  \label{fig:withdraw-exn-instance}
  \end{subfigure}

  
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.42\linewidth}
  \centering
  
  \begin{subfigure}[t]{\linewidth}
  \centering
  \begin{leancode}
|\bdef| withdraw |\returns| (history : List Nat)
|\require| balance |$\geq$| 0
|\ensures| balance + history.sum = balanceOld do
  let amounts :|\textbar| amounts.sum |$\leq$| balance
  let mut tmp := amounts
  |\whilel| tmp.nonEmpty
  |\invariant| balance    + amounts.sum = 
            balanceOld + tmp.sum 
  |\invariant| balance |$\geq$| tmp.sum 
  |\decreasing| tmp.length do
    let amount := tmp.head
    if amount > balance then 
      throw "Insufficient funds"
    else 
      balance := balance - amount
    tmp := tmp.tail
  |\lw{return}| amounts
  \end{leancode}
  \setlength{\abovecaptionskip}{16pt}
  \caption{Withdrawal with non-determinism}
  \label{fig:withdraw-nondet}
  \end{subfigure}
  
  \end{minipage}
  \setlength{\abovecaptionskip}{5pt} 
  \setlength{\belowcaptionskip}{-12pt}
  \caption{\cashmere programs featuring exceptions and non-determinism}
  \end{figure}


==> figures/withdraw_loop.tex <==

\begin{figure}[t]
  \centering
  \begin{minipage}[t]{0.48\linewidth}
  \centering
  
  \begin{subfigure}[t]{\linewidth}
  \centering
  \begin{leancode}
  |\bdef| withdraw (inAmounts : Queue Nat) |\returns| Unit
  |\ensures| balance + amounts.sum = balanceOld do
    let mut amounts := inAmounts
    |\whilel| amounts.nonEmpty
    |\invariant| balance + amounts.sum = 
      balanceOld + inAmounts.sum do
      let amount := amounts.dequeue
      balance := balance - amount
      amounts := amounts.tail
  \end{leancode}
  \caption{Balance mutation in the loop}\label{fig:withdraw-loop-partial}
  \end{subfigure}

  
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.48\linewidth}
  \centering
  
  \begin{subfigure}[t]{\linewidth}
  \centering
  \begin{leancode}
  instance : 
    MAlgOrdered (StateT Bal DivM) (Bal → Prop) where 
    |$\mu$| (f : Bal → Option (Bal → Prop) × Bal) := |$\lambda$| bl => 
      match f bl with 
      |\textbar| (some post, bl') => post bl'
      |\textbar| (none, _) => True
    ... 
    \end{leancode}
  \caption{Semantic embedding}
  \label{fig:withdraw-loop-instance}
  \end{subfigure}
  
  \end{minipage}
  
  \caption{Overview of withdrawal examples.}
  \end{figure}
  

==> figures/withdraw_state.tex <==
\begin{figure}[t]
  \centering

\begin{tabular}{cc}
  \begin{minipage}[t]{0.48\linewidth}
  \centering  
  \begin{subfigure}[t]{\linewidth}
  \centering
  \begin{leancode}
abbrev Bal := Int
def withdraw (amount : Nat) : StateM Bal Unit := do
  balance ← get 
  set (balance - amount)
  \end{leancode}
  \caption{Changing balance of the account}\label{fig:withdraw-monad}
  \end{subfigure}
  \end{minipage}
  &
    \begin{minipage}[t]{0.48\linewidth}
  \begin{subfigure}[t]{\linewidth}
  \centering
  \begin{leancode}
|\bdef| withdraw (amount : Nat) |\returns| Unit
|\ensures| balance + amount = balanceOld do
  balance := balance - amount
  \end{leancode}
  \caption{Changing balance with macros}
  \label{fig:withdraw-state}
  \end{subfigure}
  \end{minipage} 
\\\\[-8pt]
  % \vspace{1em}  
  \begin{minipage}[t]{0.48\linewidth}
  \begin{subfigure}[t]{\linewidth}
  \centering
  \begin{leancode}
instance: MAlgOrdered (StateM Bal) (Bal → Prop) where 
  |$\mu$| (f : Bal → (Bal → Prop) × Bal) := 
    |$\lambda$| b => 
      let (post, b') := f b
      post b'
  ... -- A proof that |$\mu$| is monotone 
  \end{leancode}
  \caption{Embedding stateful computations}
  \label{fig:withdraw-state-instance}
  \end{subfigure}
  \end{minipage}

  % \hfill
  % \begin{minipage}[t]{0.48\linewidth}
  % \centering

&  

  % \vspace{1em}


% |\require| balance |$\geq$| amounts.sum 

\begin{minipage}[t]{0.48\linewidth}
  \begin{subfigure}[t]{\linewidth}
    \centering
    \begin{leancode}
|\bdef| withdraw (amounts : List Nat) |\returns| Unit
|\ensures| balance + amounts.sum = balanceOld do
  let mut tmp := amounts
  |\whilel| tmp.nonEmpty
  |\invariant| balance    + amounts.sum = 
            balanceOld + tmp.sum do
    let amount := tmp.head
    balance := balance - amount
    tmp := tmp.tail
    \end{leancode}
    \caption{Session-based withdrawal loop}
    \label{fig:withdraw-loop-partial}
    \end{subfigure}
   \end{minipage}
\end{tabular}  
\setlength{\abovecaptionskip}{5pt}
\setlength{\belowcaptionskip}{-12pt}
\caption{Programming and verification in \cashmere}
\end{figure}


==> future.tex <==

\section{Future Directions}
\label{sec:future-directions}

We believe, our development of \velvet---the first foundational
multi-modal \dafny-style verifier on top of \lean---opens avenues for
several lines of exciting future work. 
%
In particular, we envision its following extensions and application,
which we are planning to explore in the future.

First, we are going to apply \velvet for specifying and verifying
computational complexity results for textbook algorithms. We believe,
in many cases, this can be achieved by enhancing the \code{VelvetM}
monad with a layer of the state monad transformer \code{StateT}, which
is supported natively by \loom~\cite{loom-paper}, and using it to
updated a counter for ``computational credits'', treating it as ghost
state.
%
We expect that in some cases, \eg, when reasoning about amortised
complexity, we will have to extend \velvet with reasoning principles
similar to that of Separation Logic with time
credits~\cite{ChargueraudP19}.
%
We are confident that this can be achieved by implementing and
specifying a set of custom operations on top of the state monad.

Another direction we are going to explore is introducing a type system
with linear capabilities on top of \velvet, thus, allowing it to
generate more SMT-friendly verification conditions, similarly to what
is achieved in tools such as Linear \dafny~\cite{LiLZCHPH22} and
\verus~\cite{verus} by means of relying on a bespoke linear type
system or by exploiting the guarantees provided by the \tname{rustc}
Rust compiler.
%
An advantage of implementing this approach on top of \velvet is that
the soundness claims similar to those of Linear \dafny and \verus can
be mechanically verified within the proof assistant, thus reducing the
trusted code base of the verifier to that of \lean.

Finally, we are planning to tackle large-scale systems verification
efforts in the style of \tname{IronFleet}~\cite{HawblitzelHKLPR15} by
making use of \emph{multiple} foundational multi-modal verifiers
implemented on top of \loom.
%
For instance, by verifying in \velvet that an implementation of a
distributed system refines its model defined in
\veil~\cite{VeilPaper}, another verifier built on top of \loom, we can
establish that all properties of the model---safety and
liveness---provably transfer to the executable implementation.
%
Furthermore, conducting such verification efforts in \lean will make
it possible to extend the state-of-the-art in trustworthy systems to a
larger class of their specifications, including information-theoretic
and security properties~\cite{probchain}.


%\is{Elaborate on the following points}

%\begin{itemize}
% \item Reasoning about program complexity;
%\item Adding linear type systems~\cite{LiLZCHPH22};
% \item Combining with \veil~\cite{VeilPaper}.
%\end{itemize}


==> internals.tex <==
\section{Implementing \velvet in \loom}
\label{sec:internals}

\velvet is built as an instance of \loom~\cite{loom-paper}---a general
and versatile \lean library for implementing provably correct
multi-modal verifiers on top of \lean by means of a monadic shallow
embedding.
%
In this section, we briefly outline the specific components of \velvet
that allow for its characteristic non-trivial features: intrinsic
verification, executable non-deterministic choice operator, an ability
to switch between reasoning about partial and total correctness, and
first-order abstractions of common data structures.

\subsection{Annotations for Intrinsic Program Verification}
\label{sec:annotations}

Under the hood, \velvet programs are ordinary \lean computations in
the \code{VelvetM} monad (see the next subsection), enriched with
specification annotations: \tlw{require}/\tlw{ensures} clauses,
assertions, loop invariants, and termination measures. 
%
These annotations are verification-only: they do not change the
executable behavior of the code. At the top level, \velvet collects
the conjunction of all \tlw{require} and \tlw{ensures} clauses into
the pre/post pair of a Hoare-style correctness statement for the
program. Likewise, loop \tlw{invariant} annotations are compiled into
hints that the verification condition generator (VCGen) can recognise.
Concretely, a loop invariant is inserted via a no-op combinator
\code{invGadget}:
%
\begin{leancodex}
|\lw{def}| invGadget (inv : Prop) : VelvetM Unit := pure ()
\end{leancodex}
%
At runtime, this expands to an idle \lean computation, but the VCGen
works over the program’s encoding and, hence, can take advantage of
the first argument of \code{invGadget} to generate appropriate
verification conditions for the loop.

\subsection{Non-Deterministic Choice Operator}
\label{sec:nondet}

As we have mentioned before, \velvet programs are computations inside
the \code{VelvetM} monad. This monad supports a non-deterministic
choice operator and divergent computations, allowing one to reason about
partial correctness. In this subsection, we will discuss the first
component. The general form of non-deterministic choice operator is:

\begin{leancodex}
|\lw{def}| pickSuchThat {|$\tau$|} (p : |$\tau$| -> Prop): VelvetM |$\tau$| := ...
\end{leancodex}

\noindent
%
This operator chooses an arbitrary value of the type $\tau$ that
satisfies the predicate \code{p}. Following \dafny-style notation, in
program code, it is written as \code{let x :|\textbar| p x}.

The weakest precondition semantics for this operator depends on the
verification style user is interested in and can be controlled. For
example, if user wants to prove that specification holds for
\emph{all} possible choices of \code{pickSuchThat}, the weakest
precondition should be a conjunction of all postconditions for the
values that satisfy the predicate \code{p}:
%
\begin{equation}
  \mathit{wp}~(\mathit{pickSuchThat}~\mathit{p})~\post = \bigwedge_{x \in p} \post~x
\end{equation}
%
Such choice operator is called ``demonic''~\cite{BroyW81} and can be
enabled by simply opening a corresponding semantics namespace
\code{open
  DemonicChoice}.
%
At the same time, the user might be interested in proving a
reachability property for the program, \ie, proving that the
specification holds for some choice of \code{pickSuchThat}. In this
case, the weakest precondition should be a disjunction of all
post-conditions for the values that satisfy the predicate and can be
enabled by \code{open AngelicChoice}.

Executing a non-deterministic choice operator is more subtle. The
problem is that \code{pickSuchThat} on its own does not provide a way
to actually choose a value from the type $\tau$ that satisfies
\code{p}. To execute computation \code{x} of type
\code{VelvetM |$\alpha$|}, \velvet implements a \code{VelvetM.run}
function which automatically tries to infer a witness of a
\code{Findable} type class for each predicate \code{p} in each
non-deterministic choice in \code{x}. Such type class provides a
recipe how to find value \code{t : |$\tau$|}, satisfying \code{p}. In
practice, instantiating \code{Findable} is rarely a problem. For
example, if \code{p} is a decidable predicate and $\tau$ is
\code{Encodable} (\ie, countable) such instance will be inferred
automatically.

\subsection{Proofs about Non-Terminating Programs}
\label{sec:termination}

Unlike vanilla \lean, where every recursive definition must carry an
explicit termination argument, \velvet decouples functional
correctness from the termination argument: a termination measure (the
\tlw{decreasing} annotation) is required only when establishing total
correctness. At the same time, for partial correctness, no such
measure is needed---the program may diverge, and proofs assert only
that, if it terminates, the postcondition holds. The user selects the
intended proof mode and the semantics of divergence---by opening the
corresponding semantic namespace, choosing between \code{open
  TotalCorrectness} to work with total correctness and \code{open
  PartialCorrectness} for partial correctness.

\velvet makes it possible to decouple proofs of partial and total
correctness. This can be done by defining two identical versions of a
program, one without termination related annotations (highlighted in
grey in~\autoref{fig:insertion-sort}) and another without functional
correctness-specific ones. The proof of the former constitutes partial
correctness, and the latter proves termination. One can then use the
following \velvet theorem to prove the program’s total correctness:
%
\begin{leancodex}
lemma partial_total_split {|$\alpha$|} : |$\forall$| (c|$_1$| c|$_2$| : VelvetM |$\alpha$|) 
  triplePartial P c|$_1$| Q → 
  (P : Prop) (Q : |$\alpha$| → Prop), eraseEq c|$_1$| c|$_2$| → 
  tripleTotal P c|$_2$| (|$\lambda$| _, True) → tripleTotal P c|$_1$| Q
\end{leancodex} 


\subsection{First-Order Abstractions of Data Structures}
\label{sec:fo-abstraction}

To make VCs amendable to SMT solvers, \velvet uses first-order (FO)
representations of \lean data structures (such as \lean arrays). The
reason is that SMT solvers are more effective on quantifier-light,
algebraic interfaces than on rich, higher-order APIs. For example, in
the insertion sort implementation from~\autoref{fig:insertion-sort} we
model arrays by the array FO theory rather than by \lean’s concrete
implementation. Such an array theory is encoded via the \code{TArray}
type class:
%
\begin{leancodex}
class TArray (|$\alpha$| : outParam Type) (|$\kappa$|: Type) where
  get : Nat → |$\kappa$| → |$\alpha$|
  set : Nat → |$\alpha$| → |$\kappa$| → |$\kappa$|
  get_set (idx|$_1$| idx|$_2$| val arr) : 
     idx|$_1$| < size arr -> get idx|$_1$| (set idx|$_2$| val arr) =
      if idx|$_1$| = idx|$_2$| then val else get idx|$_1$| arr
  ... -- other array theory operations and axioms
\end{leancodex}
%
That is, instead of implementing insertion sort taking an array
\code{a} of type \code{Array Int}, it receives \code{a} of type
\code{arrInt}, for which we assume an instance of \code{TArray Int
  arrInt}. 
%
This way, we hide the concrete implementation details from the SMT
solver: it only gets to see the abstract interface \code{TArray} where
\code{set} and \code{get} will be translated into uninterpreted
functions satisfying the array theory axioms such as \code{get_set}.

Finally, to execute programs manipulating with such array abstractions
\velvet provides a \code{TArray |$\alpha$| (Array |$\alpha$|)}
instance for arbitrary $\alpha$. It means that user can pass regular
\lean integer arrays anywhere \code{arrInt} is expected.



==> keyideas.tex <==
% **Staging the Synthesis Process: Testing Helps with Verification**
% (Key ideas)
% 1. Leveraging PBT for filtering out bad candidates
% 2. Splitting the vericoding task into smaller tasks: spec generation, impl generation, invariant synthesis, correctness proof => Loom lets you add more stages
% 3. Leveraging VC generation for invariant synthesis => smaller, easier goals (for LLMs to judge and prove)

\section{Elements of \tool Design}
\label{sec:keyideas}

This section presents the key ideas behind \tool's design.

%\vspace{-5pt}

\subsection{Staging the Synthesis Process}

%\vspace{-5pt}

Our first key idea is to stage the synthesis process by leveraging a dedicated program logic framework. Recent efforts in Lean-based vericoding typically adopt a monolithic approach: an LLM generates a complete Lean definition alongside its proof script, which is then handed directly to the prover. However, this end-to-end generation bypasses the structural advantages offered by traditional program logics. 

A prime example of this disconnect is the verification of iterative computations. In standard program verification frameworks based on Hoare logic or separation logic, loop verification is explicitly staged: the user first identifies a loop invariant, and subsequently verifies that this invariant is preserved across iterations. In contrast, a conventional Lean workflow conflates these steps. When verifying an iterative computation (whether implemented via recursive functions or monadic loops), the prover is burdened with simultaneously discovering a suitable inductive hypothesis (the functional counterpart to a loop invariant) and discharging the associated logical proof obligations. Delegating this entire verification burden to the prover in a single step fundamentally contradicts the Chain of Thought (CoT) principle.

To address this, we utilize Velvet to augment the traditional Lean vericoding pipeline with an explicit \emph{invariant inference} stage. This naturally aligns with the CoT paradigm: the LLM is first prompted to hypothesize the loop invariant independently of the proof construction. We then employ our PBT tool to conduct a preliminary check on this hypothesized invariant. If the invariant is flawed, the PBT framework immediately surfaces a concrete counterexample, guiding the LLM to iteratively refine its design before engaging in heavyweight theorem proving. Once a candidate invariant is established, the verification generator provided by Loom decomposes the overall program correctness proof into smaller, localized Verification Conditions (VCs). Before engaging in formal verification, the LLM first assesses the provability of all generated VCs and drafts informal proof sketches. If all VCs appear provable, the LLM proceeds to discharge these obligations one by one. Conversely, if any VC is deemed unprovable, this failure provides targeted feedback, guiding the LLM to backtrack and further refine the loop invariant.

\subsection{Property-Based Testing as Filters}

Our second key idea is to leverage property-based testing (PBT) as a lightweight filter to eliminate incorrect candidates early in the synthesis process. Compared to formal verification, PBT provides a cost-effective sanity check. Our PBT filter is built on top of Plausible, a property-based testing framework for Lean~4 that integrates with the tactic system. Given a theorem statement, Plausible automatically generates random test cases and attempts to refute the theorem by finding counterexamples.

\subsubsection{Handling Existential Quantification via Bounded Enumeration}

Despite its utility as a filter, PBT fundamentally struggles with existential quantification in verification tasks. While universally quantified properties can be tested by sampling inputs and checking the predicate, negating an existential post-condition requires showing that no witness exists, which in general entails reasoning over the entire domain. This severely limits the applicability of PBT in our setting. Consider the following example: given that all elements of an integer array are non-negative, prove that the sum of the array is non-negative. The theorem to test is
$(\forall i,\, i < \texttt{arr.size} \to \texttt{arr}[i] \ge 0) \to \texttt{sum}(\texttt{arr}) \ge 0$, which is logically equivalent to $(\exists i,\, i < \texttt{arr.size} \wedge \texttt{arr}[i] < 0) \vee \texttt{sum}(\texttt{arr}) \ge 0$. Plausible cannot test this directly, and such patterns are pervasive in array-related programs.

To address this, we exploit a common structural property of verification conditions: in many practical cases, existential variables admit finite bounds that can be inferred from the structure of the theorem being tested. We extend Plausible with a lightweight heuristic that analyzes the theorem structure and extracts sub-expressions appearing in inequality constraints as candidate bounds for existential variables, and uses Lean tactics (e.g., \texttt{grind}, \texttt{omega}) to prove these bounds. When such bounds can be established, we reduce existential quantification to bounded enumeration during testing, enabling effective validation that would otherwise be intractable for standard property-based testing. While this does not fully solve the challenge of testing arbitrary existential quantifiers, it covers the common patterns that arise in program verification and is effective in practice.

\subsubsection{Testing Specifications}

We use Plausible to systematically validate the generated specifications by checking their soundness and completeness. Let $I$ denotes a set of inputs. For an input $i \in I$, let $\widehat{O}(i)$ denote the set of intended outputs. A post-condition $\varphi(i, o)$ is \emph{precise} on $I$ if it satisfies: (i) \emph{soundness}---all intended outputs are accepted, i.e., $\forall i,\, \psi(i) \to \forall o \in \widehat{O}(i),\, \varphi(i, o)$; and (ii) \emph{completeness}---all unintended outputs are rejected, i.e., $\forall i,\, \psi(i) \to \forall o \notin \widehat{O}(i),\, \neg\varphi(i, o)$.

During the specification generation stage, we prompt the LLM to produce both the specification and a set of concrete test cases. Each test case consists of an input $i$ together with a representative intended output $\widehat{o} \in \widehat{O}(i)$. To validate soundness, for each test case $(i, \widehat{o})$, we use Plausible to test:
\begin{enumerate}
  \item the input satisfies the pre-condition;
  \item the input-output pair satisfies the post-condition.
\end{enumerate}
A failure in either check indicates an error in the generated specification.

Testing completeness is more challenging. However, for many algorithmic problems (e.g., typical LeetCode tasks), the intended output is deterministic, meaning $\widehat{O}(i) = \{\widehat{o}\}$. Under this assumption, testing completeness simplifies to verifying the \emph{uniqueness} of the intended output, yielding the testable form $\forall o \neq \widehat{o},\, \neg \varphi(i, o)$. Thus, checking completeness becomes a search for a spurious output $o \neq \widehat{o}$ that erroneously satisfies $\varphi$.

In practice, if a spurious output $o$ exists, it often shares a similar structure to the intended output $\widehat{o}$. We therefore adopt a combined generation strategy: we first sample candidate outputs by sampling or by applying a small mutations, then use Plausible to evaluate whether any candidate inadvertently satisfies $\varphi$. The mutations are type-directed:

\begin{itemize}
  \item \texttt{Bool}: flip the value.
  \item \texttt{Nat}: add or subtract a small constant.
  \item \texttt{Char}: add or subtract a small constant to the character code.
  \item \texttt{Int}: same as \texttt{Nat}, plus negation.
  \item $\alpha \times \beta$: mutate one components, or swap them (when $\alpha = \beta$).
  \item \texttt{Array}~$\alpha$ / \texttt{List}~$\alpha$: mutate a random element recursively, delete a random element, or insert a freshly sampled element of type $\alpha$.
  \item \texttt{String}: treated exactly as List Char.
\end{itemize}
All mutations are implemented via Lean~4 typeclasses, so multi-dimensional arrays are supported automatically through recursive instance resolution.

\subsubsection{Testing Programs and Invariants}

We further extend property-based testing to test both synthesized programs and their loop invariants. Specifically, we transform a Velvet method into a testing harness that interleaves execution with runtime checks.

Given a Velvet method:
\begin{leancodesmall}
|\lw{method}| (x : |$\alpha$|) |\lw{return}| (result : |$\beta$|)
  |\lw{requires}| pre(x)
  |\lw{ensures}| post(x, result)
  |\lw{do}|
    |\lw{while}| cond
    |\lw{invariant}| P
    |\lw{do}|
      -- loop body
    |\lw{return}| ...
\end{leancodesmall}

we construct the following testing procedure:
\begin{leancodesmall}
x |$\leftarrow$| sample(|$\alpha$|) satisfying pre(x)
if not plausible_test(P) then
    throwError "Invariant failed at entry"
|\lw{while}| cond |\lw{do}|
    -- loop body
    if not plausible_test(P) then
        throwError "Invariant not preserved"
if not plausible_test(post(x, result)) then
    throwError "Post-condition failed"
\end{leancodesmall}

Using Lean's meta-programming, we lift the Velvet monad into a testing monad that augments the original semantics with failure reporting and randomized input generation, and expose this functionality as a single Lean command, \texttt{velvet\_plausible\_test}, which runs property-based tests on Velvet methods and reports any bug along with a concrete input and the specific invariant or post-condition that was violated.

\subsection{Verification Condition Generation for Invariant Synthesis}

\todo{Summarize the key ideas of the paper here}


==> lstlean.tex <==
% Listing style definition for the Lean Theorem Prover.
% Defined by Jeremy Avigad, 2015, by modifying Assia Mahboubi's SSR style.
% Unicode replacements taken from Olivier Verdier's unixode.sty

\lstdefinelanguage{lean} {

% Anything between $ becomes LaTeX math mode
mathescape=false,
% Comments may or not include Latex commands
texcl=false,

% keywords, list taken from lean-syntax.el
morekeywords=[1]{
import, prelude, protected, private, noncomputable, definition, meta, renaming,
hiding, parameter, parameters, begin, constant, constants,
lemma, variable, variables, theory,
print, theorem, example,
open, as, export, override, axiom, axioms, inductive, with,
structure, record, universe, universes,
alias, help, precedence, reserve, declare_trace, add_key_equivalence,
match, infix, infixl, infixr, notation, postfix, prefix, instance,
eval, reduce, check, end, this,
using, using_well_founded, namespace, section,
attribute, local, set_option, extends, include, omit, class, outParam,
raw, replacing, initialize, max, default_instance,
calc, have, show, suffices, by, in, at, let, forall, Pi, fun,
if, dif, then, else, assume, obtain, from, register_simp_ext, unless, break, continue,
mutual, do, def, run_cmd, const, fix, elab, elab_rules,
partial, mut, where, macro, syntax, deriving,
return, catch, for, macro_rules, declare_syntax_cat, abbrev, 
rcases, by_cases, rintro,
% Veil
type, immutable, individual, relation, function, action, after_init,
require, assume, invariant, safety, pick, \#check_invariants_wlp,
\#check_invariants, \#check_invariants_wlp?, \#check_invariants_wlp!,
\#check_invariant_wlp, \#check_action_wlp, mut, sat, unsat, trace, bmc,
bmc_sat, any, action, actions,
%overview 
bank_def, returns, while, ensures, decreasing
},

% Sorts
morekeywords=[2]{Sort, Type, Prop, true, false, List, Nat, Bool},

% tactics, list taken from lean-syntax.el
morekeywords=[3]{
assumption, exists,
apply, intro, intros, allGoals, omega,
generalize, clear, revert, done, exact,
refine, repeat, cases, rewrite, rw,
simp, simp_all, contradiction, dsimp, trivial,
constructor, injection,
induction, try, ext,
% LeanSSr
move, sdone, sby, elim, srw, scase, shave, sapply,
=>, :,
reflect,
% Loom
mwp
},

% modifiers, taken from lean-syntax.el
% note: 'otherkeywords' is needed because these use a different symbol.
% this command doesn't allow us to specify a number -- they are put with [1]
% otherkeywords={
% [persistent], [notation], [visible], [instance], [trans_instance],
% [class], [parsing-only], [coercion], [unfold_full], [constructor],
% [reducible], [irreducible], [semireducible], [quasireducible], [wf],
% [whnf], [multiple_instances], [none], [decl], [declaration],
% [relation], [symm], [subst], [refl], [trans], [simp], [congr], [unify],
% [backward], [forward], [no_pattern], [begin_end], [tactic], [abbreviation],
% [reducible], [unfold], [alias], [eqv], [intro], [intro!], [elim], [grinder],
% [localrefinfo], [recursor]
% },

% Various symbols
literate=
{α}{{\ensuremath{\mathrm{\alpha}}}}1
{@a}{{\ensuremath{\mathrm{\alpha}}}}1
{β}{{\ensuremath{\mathrm{\beta}}}}1
{@b}{{\ensuremath{\mathrm{\beta}}}}1
{γ}{{\ensuremath{\mathrm{\gamma}}}}1
{@c}{{\ensuremath{\mathrm{\gamma}}}}1
{δ}{{\ensuremath{\mathrm{\delta}}}}1
{ε}{{\ensuremath{\mathrm{\varepsilon}}}}1
{ζ}{{\ensuremath{\mathrm{\zeta}}}}1
{η}{{\ensuremath{\mathrm{\eta}}}}1
{θ}{{\ensuremath{\mathrm{\theta}}}}1
{ι}{{\ensuremath{\mathrm{\iota}}}}1
{κ}{{\ensuremath{\mathrm{\kappa}}}}1
{μ}{{\ensuremath{\mathrm{\mu}}}}1
{ν}{{\ensuremath{\mathrm{\nu}}}}1
{ξ}{{\ensuremath{\mathrm{\xi}}}}1
{π}{{\ensuremath{\mathrm{\mathnormal{\pi}}}}}1
{ρ}{{\ensuremath{\mathrm{\rho}}}}1
{σ}{{\ensuremath{\mathrm{\sigma}}}}1
{τ}{{\ensuremath{\mathrm{\tau}}}}1
{φ}{{\ensuremath{\mathrm{\varphi}}}}1
{χ}{{\ensuremath{\mathrm{\chi}}}}1
{ψ}{{\ensuremath{\mathrm{\psi}}}}1
{ω}{{\ensuremath{\mathrm{\omega}}}}1

{∗}{{\ensuremath{\ast}}}1

{Γ}{{\ensuremath{\mathrm{\Gamma}}}}1
{Δ}{{\ensuremath{\mathrm{\Delta}}}}1
{Θ}{{\ensuremath{\mathrm{\Theta}}}}1
{Λ}{{\ensuremath{\mathrm{\Lambda}}}}1
{Σ}{{\ensuremath{\mathrm{\Sigma}}}}1
{Φ}{{\ensuremath{\mathrm{\Phi}}}}1
{Ξ}{{\ensuremath{\mathrm{\Xi}}}}1
{Ψ}{{\ensuremath{\mathrm{\Psi}}}}1
{Ω}{{\ensuremath{\mathrm{\Omega}}}}1

{ℵ}{{\ensuremath{\aleph}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1
{≠}{{\ensuremath{\neq}}}1
{≈}{{\ensuremath{\approx}}}1
{≡}{{\ensuremath{\equiv}}}1
{≃}{{\ensuremath{\simeq}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1

{∂}{{\ensuremath{\partial}}}1
{∆}{{\ensuremath{\triangle}}}1 % or \laplace?

{∫}{{\ensuremath{\int}}}1
{∑}{{\ensuremath{\mathrm{\Sigma}}}}1
{Π}{{\ensuremath{\mathrm{\Pi}}}}1

{⊥}{{\ensuremath{\perp}}}1
{∞}{{\ensuremath{\infty}}}1
{∂}{{\ensuremath{\partial}}}1

{∓}{{\ensuremath{\mp}}}1
{±}{{\ensuremath{\pm}}}1
{×}{{\ensuremath{\times}}}1

{⊕}{{\ensuremath{\oplus}}}1
{⊗}{{\ensuremath{\otimes}}}1
{⊞}{{\ensuremath{\boxplus}}}1

{∇}{{\ensuremath{\nabla}}}1
{√}{{\ensuremath{\sqrt}}}1

{⬝}{{\ensuremath{\cdot}}}1
{•}{{\ensuremath{\cdot}}}1
{∘}{{\ensuremath{\circ}}}1

%{⁻}{{\ensuremath{^{\textup{\kern1pt\rule{2pt}{0.3pt}\kern-1pt}}}}}1
{⁻}{{\ensuremath{^{-}}}}1
{▸}{{\ensuremath{\blacktriangleright}}}1

{∧}{{\ensuremath{\wedge}}}1
{∨}{{\ensuremath{\vee}}}1
{¬}{{\ensuremath{\neg}}}1
{⊢}{{\ensuremath{\vdash}}}1

%{⟨}{{\ensuremath{\left\langle}}}1
%{⟩}{{\ensuremath{\right\rangle}}}1
{⟨}{{\ensuremath{\langle}}}1
{@langle}{{\ensuremath{\langle}}}1
{⟩}{{\ensuremath{\rangle}}}1

{↦}{{\ensuremath{\mapsto}}}1
{←}{{\ensuremath{\leftarrow}}}1
%{<-}{{\ensuremath{\leftarrow}}}1
{→}{{\ensuremath{\rightarrow}}}1
{↔}{{\ensuremath{\leftrightarrow}}}1
{<->}{{\ensuremath{\leftrightarrow}}}1
{⇒}{{\ensuremath{\Rightarrow}}}1
{⟹}{{\ensuremath{\Longrightarrow}}}1
{⇐}{{\ensuremath{\Leftarrow}}}1
{⟸}{{\ensuremath{\Longleftarrow}}}1


{∩}{{\ensuremath{\cap}}}1
{∪}{{\ensuremath{\cup}}}1
{⊂}{{\ensuremath{\subseteq}}}1
{⊆}{{\ensuremath{\subseteq}}}1
{⊄}{{\ensuremath{\nsubseteq}}}1
{⊈}{{\ensuremath{\nsubseteq}}}1
{⊃}{{\ensuremath{\supseteq}}}1
{⊇}{{\ensuremath{\supseteq}}}1
{⊅}{{\ensuremath{\nsupseteq}}}1
{⊉}{{\ensuremath{\nsupseteq}}}1
{∈}{{\ensuremath{\in}}}1
{∉}{{\ensuremath{\notin}}}1
{∋}{{\ensuremath{\ni}}}1
{∌}{{\ensuremath{\notni}}}1
{∅}{{\ensuremath{\emptyset}}}1

{∖}{{\ensuremath{\setminus}}}1
{†}{{\ensuremath{\dag}}}1

{ℕ}{{\ensuremath{\mathbb{N}}}}1
{ℤ}{{\ensuremath{\mathbb{Z}}}}1
{ℝ}{{\ensuremath{\mathbb{R}}}}1
{ℚ}{{\ensuremath{\mathbb{Q}}}}1
{ℂ}{{\ensuremath{\mathbb{C}}}}1
{⌞}{{\ensuremath{\llcorner}}}1
{⌟}{{\ensuremath{\lrcorner}}}1
{⦃}{{\ensuremath{\{\!|}}}1
{⦄}{{\ensuremath{|\!\}}}}1

{‖}{{\ensuremath{\|}}}1
{₁}{{\ensuremath{_1}}}1
{₂}{{\ensuremath{_2}}}1
{₃}{{\ensuremath{_3}}}1
{₄}{{\ensuremath{_4}}}1
{₅}{{\ensuremath{_5}}}1
{₆}{{\ensuremath{_6}}}1
{₇}{{\ensuremath{_7}}}1
{₈}{{\ensuremath{_8}}}1
{₉}{{\ensuremath{_9}}}1
{₀}{{\ensuremath{_0}}}1
{ᵢ}{{\ensuremath{_i}}}1
{ⱼ}{{\ensuremath{_j}}}1
{ₐ}{{\ensuremath{_a}}}1

{¹}{{\ensuremath{^1}}}1

{ₙ}{{\ensuremath{_n}}}1
{ₘ}{{\ensuremath{_m}}}1
{ₚ}{{\ensuremath{_p}}}1
{↑}{{\ensuremath{\uparrow}}}1
{↓}{{\ensuremath{\downarrow}}}1

{...}{{\ensuremath{\ldots}}}1
{·}{{\ensuremath{\cdot}}}1

{▸}{{\ensuremath{\triangleright}}}1

{Σ}{{\color{symbolcolor}\ensuremath{\Sigma}}}1
{Π}{{\color{symbolcolor}\ensuremath{\Pi}}}1
{∀}{{\color{symbolcolor}\ensuremath{\forall}}}1
{@all}{{\color{symbolcolor}\ensuremath{\forall}}}1
{@ex}{{\color{symbolcolor}\ensuremath{\exists}}}1
{∃}{{\color{symbolcolor}\ensuremath{\exists}}}1
{λ}{{\color{symbolcolor}\ensuremath{\mathrm{\lambda}}}}1
{\$}{{\color{symbolcolor}\$}}1

{:=}{{\color{symbolcolor}:=}}1
{=}{{\color{symbolcolor}=}}1
{//}{{\color{symbolcolor}//}}1
{/}{{\color{symbolcolor}/}}1
{<|>}{{\color{symbolcolor}<|>}}1
{|>}{{\ensuremath{\triangleright}}}1
{<\$>}{{\color{symbolcolor}<\$>}}1
{+}{{\color{symbolcolor}+}}1
{*}{{\color{symbolcolor}*}}1,

% Comments
%comment=[s][\itshape \color{commentcolor}]{/-}{-/},
morecomment=[s][\color{commentcolor}]{/-}{-/},
morecomment=[l][\itshape \color{commentcolor}]{--},

% Spaces are not displayed as a special character
showstringspaces=false,

% keep spaces
keepspaces=true,

% String delimiters
morestring=[b]",
morestring=[d],

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=false,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,
breakatwhitespace=true,

% Default style fors listingsred
basicstyle=\ttfamily\small,

% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]fullflexible,


% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the beginning of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{keywordcolor}},

% Style for sorts
keywordstyle=[2]{\ttfamily\color{sortcolor}},

% Style for tactics keywords
keywordstyle=[3]{\ttfamily\color{tacticcolor}},

% Style for attributes
keywordstyle=[4]{\ttfamily\color{attributecolor}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle={\ttfamily\footnotesize },

}
